On Quality of Monitoring for Multi-channel Wireless Infrastructure Networks

Passive monitoring utilizing distributed wireless sniffers is an effective technique to monitor activities in wireless infrastructure networks for fault diagnosis, resource management and critical path analysis. In this paper, we introduce a quality of monitoring (QoM) metric defined by the expected number of active users monitored, and investigate the problem of maximizing QoM by judiciously assigning sniffers to channels based on the knowledge of user activities in a multi-channel wireless network. Two types of capture models are considered. The user-centric model assumes frame-level capturing capability of sniffers such that the activities of different users can be distinguished while the sniffer-centric model only utilizes the binary channel information (active or not) at a sniffer. For the user-centric model, we show that the implied optimization problem is NP-hard, but a constant approximation ratio can be attained via polynomial complexity algorithms. For the sniffer-centric model, we devise stochastic inference schemes to transform the problem into the user-centric domain, where we are able to apply our polynomial approximation algorithms. The effectiveness of our proposed schemes and algorithms is further evaluated using both synthetic data as well as real-world traces from an operational WLAN.

==> TMC arxiv submission/Commands.tex <==
%!TEX root = MultiAgentBandit.tex
%\usepackage[textwidth=18\marginparwidth]{todonotes}

%\usepackage{pdfsync}
%% For citations
%\usepackage{natbib}
%%\bibliographystyle{apalike}
%
%\if0
%\newcommand{\citep}[1]{\cite{#1}}
%\newcommand{\citet}[1]{\cite{#1}}
%\newcommand{\citealt}[1]{\cite{#1}}
%\newcommand{\iftextcite}[1]{}
%
%\newcommand{\npcite}[1]{\cite{#1}}
%\newcommand{\yrcite}[1]{\cite{#1}}
%\fi


%\usepackage{algorithm}
%\usepackage[vlined,algonl,boxed]{algorithm2e}
\usepackage[ruled,vlined]{algorithm2e}
\usepackage{algpseudocode}

%\usepackage{amsthm}

\usepackage{amssymb}
\usepackage{array}
%\usepackage[dvips]{graphics}
\usepackage{amsmath} % Learn about the AMS package, again very useful!
%\usepackage{color}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{stmaryrd}
%\usepackage{algorithm,algorithmic}
%\usepackage{dsfont}
\usepackage{subfig}
\usepackage{paralist}
%\usepackage{small-headings}
\usepackage{verbatim}

\usepackage{framed}
\usepackage[dvipsnames]{color}
\definecolor{shadecolor}{gray}{0.85}

\usepackage{soul}
\newcommand{\GS}[1]{\hl{GS: #1}}
\newcommand{\RZ}[1]{\hl{RZ: #1}}

\newif\iflong % Sometimes we want to keep two versions; a short and a long one -- this is useful for that..
\longfalse
%\longtrue

\newif\ifcomm
%\commfalse
\commtrue

% THEOREMS -------------------------------------------------------
\newtheorem{thm}{Theorem}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{proofthm}{Proof of Theorem 2}
\newtheorem{defn}{Definition}
\newtheorem{rem}[thm]{Remark}
\newtheorem{ex}[thm]{Example}
\newtheorem{remark}{Remark}

% MATH -----------------------------------------------------------
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\rationals}{\mathbb{Q}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\naturals}{\mathbb{N}}
\newcommand{\unitstep}{\mathbb{U}}
\newcommand{\eps}{\varepsilon}
\newcommand{\To}{\longrightarrow}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\partialderiv}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\ds}{\displaystyle}
\newcommand{\argmin}{\arg\min}
\newcommand{\argmax}{\arg\max}
\newcommand{\sq}{\hbox{\rlap{$\sqcap$}$\sqcup$}}
\DeclareMathOperator{\maxstep}{maxstep}

\newcommand{\smallnorm}[1]{\|#1\|}
\newcommand{\supnorm}[1]{\norm{#1}_\infty}
\newcommand{\cset}[2]{\left\{\,#1\,:\,#2\,\right\}}
\renewcommand{\natural}{\mathbb N}                   % Natural numbers
\newcommand{\Real}{\mathbb R}                        % Real numbers
\newcommand{\real}{\mathbb R}                        % again..
\newcommand{\R}{{\mathbb{R}}}                        % again..

\newcommand{\Prob}[1]{{\mathbb P}\left(#1\right)}    % Probabilities; example: \Prob{X>\eps}<1-\delta
\renewcommand{\P}{{\mathbb P}}                         % Probabilities when we want to control the parenthesis
\newcommand{\EE}[1]{{\mathbb E}\left[#1\right]}      % Expectations
\newcommand{\E}{{\mathbb E}}                         % Expectations  when we want to control the parenthesis
\newcommand{\Var}[1]{{\mathrm{Var}}\left[#1\right]}  % Variances
%\newcommand{\one}{\mathbb I}
\newcommand{\one}[1]{{\mathbb I}_{\{#1\}}}           % Characteristic function

\newcommand{\scons}{$s$-constraint}
\newcommand{\ucons}{$u$-constraint}

\newcommand{\mec}{MEC}
\newcommand{\tsat}{3SAT}
\newcommand{\montsat}{MON3SAT}
\newcommand{\mcgbc}{MC-GBC}
\newcommand{\greedy}{Greedy}
\newcommand{\opt}{OPT}
\newcommand{\probrand}{ProbRand}
\newcommand{\piperand}{PipeRand}
\newcommand{\pbar}{\overline{p}}

%\newcommand{\mec}{{\sc mec}}
%\newcommand{\tsat}{{\sc 3sat}}
%\newcommand{\montsat}{{\sc monotone-3sat}}
%\newcommand{\mcgbc}{{\sc mc-gbc}}
%\newcommand{\greedy}{{\sc Greedy}}
%\newcommand{\opt}{{\sc Opt}}
%\newcommand{\probrand}{{\sc ProbRand}}
%\newcommand{\piperand}{{\sc PipeRand}}

\newenvironment{proof-sketch}{{\noindent\em Proof Sketch.}\hspace*{0.3em}}{\hfill\QED\medskip}
%\newenvironment{proof}{{\bf Proof.}}{\hfill\rule{2mm}{2mm}\\}
\newenvironment{proof-of}[1]{{\noindent\em Proof of #1.}\hspace*{0.3em}}{\hfill\qed\medskip}



\newcounter{assumption}%[section]
\newcommand{\theassumptionletter}{A}
\renewcommand{\theassumption}{\theassumptionletter\arabic{assumption}}

\newenvironment{ass}[1][]{\begin{trivlist}\item[] \refstepcounter{assumption}%
 {\bf Assumption\ \theassumption\ #1} }{%\par\nobreak\noindent\sl\ignorespaces}{%
 \ifvmode\smallskip\fi\end{trivlist}}
\newcommand{\aref}[1]{(\ref{#1})}



% Keep whatever you need from here

\newcommand{\MB}{\mathcal{B}}
\newcommand{\MA}{\mathcal{A}}
\newcommand{\MS}{\mathcal{S}}
\newcommand{\MF}{\mathcal{F}}
\newcommand{\MC}{\mathcal{C}}
\newcommand{\MRR}{\mathcal{R}}
\newcommand{\MD}{\mathcal{D}}
\newcommand{\MP}{\mathcal{P}}
\newcommand{\MU}{\mathcal{U}}
\newcommand{\MO}{\mathcal{O}}
\newcommand{\MX}{\mathcal{X}}
\newcommand{\GG}{\mathcal{G}}
\newcommand{\hZ}{\hat{Z}}
\newcommand{\hF}{\hat{F}}
\newcommand{\hL}{\hat{L}}
\newcommand{\tL}{\tilde{L}}

\newcommand{\MI}{{\bf I}} %\mathbb{I}}


\newcommand{\ep}{\varepsilon}                        % Shorthand for nice epsilon
\newcommand{\de}{\delta}                             % Shorthand for delta
\newcommand{\ra}{\rightarrow}
\newcommand{\diag}{\mathop{\rm diag}}
\newcommand{\inlinemin}{\wedge}
\newcommand{\inlinemax}{\vee}

\newcommand{\ip}[2]{\langle #1,#2 \rangle}
\newcommand{\eqdef}{\stackrel{\mbox{\rm\tiny def}}{=}}
\newcommand{\aP}{{\cal P}}

% Shorthands I use for math environments
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\beqan}{\begin{eqnarray*}}
\newcommand{\eeqan}{\end{eqnarray*}}
\newcommand{\ben}{\begin{eqnarray*}}
\newcommand{\een}{\end{eqnarray*}}

\newcommand{\RA}{$\Rightarrow$}
\ifcomm
   \newcommand\comm[1]{\textcolor{blue}{ #1}}
\else
   \newcommand\comm[1]{}
   \renewcommand{\todo}[1]{}
\fi
\newcommand{\remove}[1]{\textcolor{blue}{\sout{#1}}}
\newcommand{\tO}{\tilde{O}}

% Boldfaced lowercase greek letters as described at
% http://www.rpi.edu/dept/acs/rpinfo/common/Computing/Consulting/Software/LaTeX/Hints/Greek_Chars.html
\def\bmath#1{\mbox{\boldmath$#1$}}
% http://www.ctan.org/tex-archive/info/symbols/comprehensive/symbols-a4.pdf page 68
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

\newcommand{\bm}{\boldmath}
%\newcommand{\beq}{\begin{equation}}
%\newcommand{\eeq}{\end{equation}}
\newcommand{\Nbar}{\bar N}
\newcommand{\lra}{\longrightarrow}
\newcommand{\lla}{\longleftarrow}
\newcommand{\mc}{\multicolumn}
%\newcommand{\qed}{{\hfill$\Box$}}
\newcommand{\C}{\mbox{\bm $C$}}
\newcommand{\Cs}{\mbox{\scriptsize\bm $C$}}
\newcommand{\cc}{\mbox{\bm $c$}}
\newcommand{\bb}{\mbox{\bm $b$}}
\newcommand{\m}{\mbox{\bm $m$}}
\newcommand{\PP}{\mbox{\bm $P$}}
\newcommand{\uu}{\mbox{\bm $u$}}
\newcommand{\Gg}{\mbox{\bm $g$}}
\newcommand{\ccc}{{\bf c}}
\newcommand{\sss}{\mbox{$\mathbf{s}$}}
\newcommand{\xx}{\mbox{$\mathbf{x}$}}
\newcommand{\pp}{\mbox{$\mathbf{p}$}}
\newcommand{\xxx}{{\bm x}}
\newcommand{\rr}{\mbox{\bm $r$}}
\newcommand{\Z}{\mbox{\bm $Z$}}
\newcommand{\0}{{\bf 0}}
\newcommand{\N}{{\cal N}}
\newcommand{\zero}{\mbox{\bm  $0$}}
\newcommand{\vv}{\mbox{\bm $v$}}
\newcommand{\vvb}{\mbox{\scriptsize\bm $v$}}
\newcommand{\yy}{\mbox{$\mathbf y$}}
\newcommand{\G}{\mbox{\bm $G$}}
\renewcommand{\L}{\mbox{\bm $L$}}
\newcommand{\I}{\mbox{\bm $I$}}
\newcommand{\A}{\mbox{\bm $A$}}
\newcommand{\B}{\mbox{\bm $B$}}
\newcommand{\T}{\mbox{\bm $T$}}
\newcommand{\X}{\mbox{\bm $X$}}
\newcommand{\Y}{\mbox{\bm $Y$}}
\newcommand{\bydef}{{\buildrel{\triangle}\over =}}
\newcommand{\tht}{\theta}
\newcommand{\Zhat}{{\hat Z}}
\newcommand{\yhat}{{\hat y}}
\newcommand{\dbar}{{\bar d}}
\newcommand{\cund}{{\underline c}}
\newcommand{\Nhat}{{\hat N}}
\newcommand{\mubar}{{\bar\mu}}
\newcommand{\sigmahat}{{\hat \sigma}}
\newcommand{\sigmabar}{{\bar \sigma}}
\newcommand{\si}{{\sigma}}
\newcommand{\rhohat}{{\hat \rho}}
\newcommand{\thetahat}{{\hat \theta}}
\newcommand{\xb}  {{\mbox{\boldmath $x$}}}
\newcommand{\vb}  {{\mbox{\boldmath $v$}}}
\newcommand{\mem}[1]{\label{eq:#1}}
\newcommand{\rec}[1]{(\ref{eq:#1})}
\newcommand{\nono}{\nonumber}
\newcommand{\scc}{{\cal S}}
\newcommand{\yc}{{\cal C}}
\newcommand{\MK}{{\cal K}}
\newcommand{\Cb}  {{\mbox{\boldmath $C$}}}

\newcommand{\profit}[1]{\sum_{u \in #1} p_u}
\newcommand{\half}{\frac{1}{2}}

\newcommand{\qlica}{{\sc qlICA}}
\newcommand{\bica}{{\sc bICA}}

